Detection of Lying Electrical Vehicles in Charging Coordination Application Using Deep Learning

The simultaneous charging of many electric vehicles (EVs) stresses the distribution system and may cause grid instability in severe cases. The best way to avoid this problem is by charging coordination. The idea is that the EVs should report data (such as state-of-charge (SoC) of the battery) to run a mechanism to prioritize the charging requests and select the EVs that should charge during this time slot and defer other requests to future time slots. However, EVs may lie and send false data to receive high charging priority illegally. In this paper, we first study this attack to evaluate the gains of the lying EVs and how their behavior impacts the honest EVs and the performance of charging coordination mechanism. Our evaluations indicate that lying EVs have a greater chance to get charged comparing to honest EVs and they degrade the performance of the charging coordination mechanism. Then, an anomaly based detector that is using deep neural networks (DNN) is devised to identify the lying EVs. To do that, we first create an honest dataset for charging coordination application using real driving traces and information revealed by EV manufacturers, and then we also propose a number of attacks to create malicious data. We trained and evaluated two models, which are the multi-layer perceptron (MLP) and the gated recurrent unit (GRU) using this dataset and the GRU detector gives better results. Our evaluations indicate that our detector can detect lying EVs with high accuracy and low false positive rate.

==> Bio/bio.tex <==
%\newpage
\section*{Biographies}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/Ahmed_Shafee.jpg}}]{Ahmed A. Shafee}
	is currently a Graduate Teaching Assistant in the Department of Electrical \& Computer Engineering, Tennessee Tech. University, USA and pursuing his Ph.D. degree in the same department.
	He received the B.S. degree and the M.S. degree in Computer Engineering from Helwan University, Cairo, Egypt in 2011 and 2018, respectively.
	His research interests include machine learning, artificial intelligence, intrusion detection, cryptography and network security, smart-grid and AMI networks, and electric vehicles.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/mfouda.jpg}}]{Mostafa M. Fouda} (SM'14) is currently an associate professor at Benha University (Egypt), and an adjunct graduate faculty member at Tennessee Technological University (USA). He is also a former assistant professor at Tohoku University (Japan). Dr. Fouda received his B.S. (with Hons.) and M.S. degrees from Benha University (Egypt) in 2002 and 2007, respectively, and his Ph.D. degree from Tohoku University (Japan) in 2011. He has published over 30 papers mostly in IEEE conference proceedings and journals. His research has been cited more than 1200 times. He has served on the technical committees of several IEEE conferences such as IEEE ICC, GLOBECOM, etc. He is also a reviewer in several IEEE Transactions/Magazines and an associate editor of IEEE Access.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/mohamed_mahmoud.jpg}}]{Mohamed M. E. A. Mahmoud}
	received PhD degree from the University of Waterloo in April 2011. From May 2011 to May 2012, he worked as a postdoctoral fellow in the Broadband Communications Research group - University of Waterloo. From August 2012 to July 2013, he worked as a visiting scholar in University of Waterloo, and a postdoctoral fellow in Ryerson University. Currently, Dr Mahmoud is an associate professor in Department Electrical and Computer Engineering, Tennessee Tech University, USA. The research interests of Dr. Mahmoud include security and privacy preserving schemes for smart grid communication network, mobile ad hoc network, sensor network, and delay-tolerant network. Dr. Mahmoud has received NSERC-PDF award. He won the Best Paper Award from IEEE International Conference on Communications (ICC'09), Dresden, Germany, 2009. Dr. Mahmoud is the author for more than twenty three papers published in major IEEE conferences and journals, such as INFOCOM conference and IEEE Transactions on Vehicular Technology, Mobile Computing, and Parallel and Distributed Systems. He serves as an Associate Editor in Springer journal of peer-to-peer networking and applications. He served as a technical program committee member for several IEEE conferences and as a reviewer for several journals and conferences such as IEEE Transactions on Vehicular Technology, IEEE Transactions on Parallel and Distributed Systems, and the journal of Peer-to-Peer Networking.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/Waleed.jpg}}]{Waleed Alasmary}(SM'19) received the B.Sc. degree (Hons.) in computer engineering from Umm Al-Qura University, Saudi Arabia, in 2005, the M.A.Sc. degree in electrical and computer engineering from the University of Waterloo, Canada, in 2010, and the Ph.D. degree in electrical and computer engineering from the University of Toronto, Toronto, Canada, in 2015. During his Ph.D. degree, he was a Visiting Research Scholar with Network Research Laboratory, UCLA, in 2014. He was a Fulbright Visiting Scholar with CSAIL Laboratory, MIT, from 2016 to 2017. He subsequently joined the College of Computer and Information Systems, Umm Al-Qura University, as an Assistant Professor of computer engineering. His ``Mobility impact on the IEEE 802.11p'' article is among the most cited Ad Hoc Networks journal articles list from 2016-2018. He published articles in prestigious conferences and journals, such as the IEEE Transactions on Vehicular Technology and the IEEE Communications Surveys and Tutorials. His current research interests include mobile computing, ubiquitous sensing, and intelligent transportation systems, privacy and anonymity.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/abdulah-uos.jpg}}]{Abdulah Jeza Aljohani}  received the B.Sc (Eng.) degree in electronics and communication engineering from King Abdulaziz University, Jeddah, Saudi Arabia, in 2006, and the M.Sc. degree with distinction and Ph.D. degree, in wireless communication from the University of Southampton, Southampton, U.K., in 2010 and 2016, respectively. He is currently an Assistance Professor with the Center of Excellence in Intelligent Engineering Systems and the Department of Electrical and Computer Engineering, King Abdulaziz University, Jeddah, Saudi Arabia. He is also associated with Center
of Excellence in Intelligent Engineering Systems (CEIES), KAU. His research interests include joint source/channel coding, distributed source coding, coded modulation, channel coding, cooperative communications, and MIMO systems.
\end{IEEEbiography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/Fathi_Amsaad.jpg}}]{Fathi Amsaad} is an Assistant Professor in the School of Information Security and Applied Computing (SISAC) at Eastern Michigan University (EMU). From August 2018 to August 2019, he was an Assistant Professor in the University of Southern Mississippi (USM), Hattiesburg, MS, USA. From August 2016 to August 2017, he was a Visiting Instructor with the University of South Florida (USF), Tampa, FL, USA. From August 2014 to August 2016 he worked as an Adjunct Instructor at Bowling Green State University (BGSU), Ohio, USA. From August 2012 to August 2016, he was a Graduate Assistant (Teaching Assistant, Research Assistant, and Instructor) at the University of Toledo, Ohio, USA. 
Prior coming to North America, he received a B. Sc. in Computer Science from the top ranked University in Libya, the University of Benghazi, Libya, and worked as a teaching assistant and the senior project lab administrator in the University. 
He worked as a Network and Security Engineer for several year prior coming to USA. 
In 2012, he received a dual Master of Science Degree in Computer Science/ Computer Engineering, with two Professional Certificates in Networking and Advanced Programming, from University of Bridgeport, CT. He also received a Ph.D. degree in Engineering, with an emphasis in Computer Science and Engineering, from the University of Toledo, Ohio, USA, in Dec. 2017. 
His research interests are in the area of Cyber and Physical Systems Security with special interest in Hardware Oriented Security and Trust for Embedded and Smart Systems Security, Security of IoT Applications, and AMI and Autonomous Systems Cybersecurity. He served as a session chair and member for several IEEE conferences and as a reviewer for several journals and conferences such as IEEE IoT Journal, IEEE Access Journal, IEEE ISCAS conference and MDPI Journals. He received the prestigious IEEE Best Graduate Student Award, from IEEE and College of Engineering, University of Toledo, Ohio and was nominee for the best Ph.D. Dissertation Award. 

\end{IEEEbiography}

